Multimodal graph representation learning for website generation based on visual sketch

The Design2Code problem, which involves converting digital designs into functional source code, is a significant challenge in software development due to its complexity and time-consuming nature. Traditional approaches often struggle with accurately interpreting the intricate visual details and structural relationships inherent in webpage designs, leading to limitations in automation and efficiency. In this paper, we propose a novel method that leverages multimodal graph representation learning to address these challenges. By integrating both visual and structural information from design sketches, our approach enhances the accuracy and efficiency of code generation, particularly in producing semantically correct and structurally sound HTML code. We present a comprehensive evaluation of our method, demonstrating significant improvements in both accuracy and efficiency compared to existing techniques. Extensive evaluation demonstrates significant improvements of multimodal graph learning over existing techniques, highlighting the potential of our method to revolutionize design-to-code automation. Code available at https://github.com/HySonLab/Design2Code

==> chapters/31_methodology.tex <==
    \subsection{Multimodal graph-based learning} \label{sec:multimodal-graph}
    For the basic architecture of the model, we adapt the Flamingo model, a vision-language model designed for various forms of image media such as videos and images. This established the model to handle graph-based inputs.
    
    \paragraph{Extract embeddings by Vision Encoder.} We utilize the ViT-L-14 backbone to extract vision embeddings. These embeddings are then passed through the Perceiver Resampler module, where the data is reshaped to be compatible with other components of the model.

    \begin{figure*}[t]
        \centering
        \includegraphics[width=1\linewidth]{graphics/gc_att.pdf}
        \caption{Detail of the fusion process of multiple modalities within the Flamingo Language layer}
        \label{fig:fusion_lm}
    \end{figure*}
    
    \paragraph{Reducing embedding-size by Perceiver Resampler.} The \textit{Perceiver Resampler} is a crucial module that connects varying-sized visual features to the pre-trained language model. This module is inspired by the \textbf{Perceiver} architecture by Jaegle et al. (2021). The Perceiver is a Transformer-based architecture designed to efficiently handle inputs from various modalities, including images, audio, and text. It employs an attention mechanism to process inputs of varying sizes and transforms them into fixed-size outputs. Specifically, this module resamples the input features from varying sizes into a fixed set of tokens (e.g., 64 tokens). The reason for this is to reduce computational complexity during cross-attention between images and text, as the number of visual tokens is fixed, regardless of the original size of the visual features. Operationally, this module learns a fixed number of latent input queries as embeddings. These latent input queries are then used to perform cross-attention with the flattened visual features generated by the vision encoder. The result of the cross-attention is a fixed set of visual tokens, for instance, 64 tokens.

    
    \paragraph{Encoding geometric information by Graph Convolutional Network.} In addition to the image encoder, we employ a basic Graph Convolutional Network (GCN) to encode information from the graph. Specifically, GCN receives input as nodes and edges from the graph, and then performs information propagation through convolutional layers to generate embeddings that represent each node. These embeddings contain information about the relationships and attributes of the nodes within the graph.

    \paragraph{Preprocessing text input.} To ensure training consistency with the original Flamingo model, we add a special tag, \texttt{<graph>}, at the beginning, alongside \texttt{<image>}, to enable accurate cross-attention. Specifically, this allows the graph embedding to cross-attend correctly with the text embedding. For example,
    \begin{itemize}
        \item For the initial text: \texttt{<html> ... </html>}
        \item After prepending the necessary tokens such as the \texttt{<graph>} token, the text is: \texttt{<graph> <image> <html> ... </html> <sos>}
    \end{itemize}  

    
    \paragraph{Fusion of Graph and Vision Context with Language in Flamingo Layer.} In the Flamingo Layer, we proposed a method that involves incorporating features from the graph modality through cross attention between two pairs of modalities: vision with text and vision with graph. The demonstration is shown through \ref{fig:model}
    \begin{itemize}
        % \item \textbf{Input:} The inputs are semantic vectors from descriptive sentences (\texttt{lang\_x}), visual features (\texttt{vis\_x}), and graph information (\texttt{graph\_x}). These inputs are fed into the Gated Cross-Attention layer to fuse the modalities.
        \item \textbf{Model Training Inputs:}
            \begin{itemize}
                \item \textbf{Image:} The image is converted into visual features $\mathbf{X}$ using the Flamingo Vision Encoder.
                \item \textbf{Graph:} In this case, the graph can represent the relationships between objects in the image and their components. For example, it may include nodes and edges representing objects such as "Button", "Title", and their relationships.
            \end{itemize}
        \item To perform fusion, we first apply cross attention between the vision and text modalities, and then perform attention between graph embeddings and text embeddings. After completing the embeddings, we combine the outputs of the two cross attentions with a shortcut connection. The process is given by the formula:
        \begin{equation}
            \mathbf{E}_{\text{L}}^i = \text{GCA}(\mathbf{X},  \mathbf{E}_\text{L}^{i-1}) +  \text{GCA}(\mathbf{Z}, \mathbf{E}_\text{L}^{i-1})  + \mathbf{E}_\text{L}^{i-1}
        \end{equation}
        where $\mathbf{X}$, $\mathbf{Z}$ are the vision embedding and the graph embedding, correspondingly. $\mathbf{E}_\text{L}^{i}$ is the language output from the $i$-th Flamingo Layer, which fuses graph and vision into text embedding. The first layer receives $\mathbf{E}_\text{L}^{0} = \mathbf{Y}$, which is the initial text embedding. $\text{GCA}(\mathbf{A}, \mathbf{B})$ denotes the Gated Cross-Attention operator that performs attention between two embeddings $\mathbf{A}$ and $\mathbf{B}$ from different modalities.
    
        \item The model applies attention techniques to combine information from text with information from HTML design and graphs. For example, the model may learn to link visual components such as "button" with text representing the code "button" in HTML and adjacent blocks in the graph to determine the position and layout of the button in the overall structure of the webpage. The use of a gated mechanism helps the model decide which parts of the visual and graph information are crucial for generating descriptive text.
    \end{itemize}


    
% -------------------------------------------------------------------------
    \subsection{Code Generation} 
    During inference, we construct a graph from the initial image and set up the initial prompt tokens for inference. In this case, we use the \texttt{<html>} token as the initial prompt token to subsequently build the design code. These tokens are then fed into the decoder for inference.
    To summary, in the inference stage, we execute over three stages:
    \begin{enumerate}
        \item First, export components for the graph using the method mentioned in Section \ref{sec:graph_construct}.
        \item Then, prepend the token \texttt{<html>} as the initial token for further generation.
        \item Finally, use the graph encoding and vision encoding to encode the whole image and the graph exported from the image. This is fused with the language decoder to complete the code generation.
        \end{enumerate}

